Large-eddy simulations with ClimateMachine: a new open-source code for atmospheric simulations on GPUs and CPUs

We introduce ClimateMachine, a new open-source atmosphere modeling framework using the Julia language to be performance portable on central processing units (CPUs) and graphics processing units (GPUs). ClimateMachine uses a common framework both for coarser-resolution global simulations and for high-resolution, limited-area large-eddy simulations (LES). Here, we demonstrate the LES configuration of the atmosphere model in canonical benchmark cases and atmospheric flows, using an energy-conserving nodal discontinuous-Galerkin (DG) discretization of the governing equations. Resolution dependence, conservation characteristics and scaling metrics are examined in comparison with existing LES codes. They demonstrate the utility of ClimateMachine as a modelling tool for limited-area LES flow configurations.

==> macros.tex <==
% \usepackage[T1]{fontenc}
% \usepackage[utf8]{inputenc}
% \usepackage{times}

% \usepackage[font=small,labelfont=bf,tableposition=top]{caption}
% \usepackage{graphicx}
% \usepackage{natbib} 
\usepackage{bm}
% \usepackage{verbatim}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{color, soul}
% \usepackage{hyperref}
% %\usepackage{algorithmicx}
% \usepackage{algpseudocode}
\usepackage{subcaption}
\usepackage{stackengine} %for subfigures without a, b, c ...
% \usepackage{stmaryrd}
% \usepackage{appendix}

\renewcommand{\vec}[1]{\boldsymbol{{#1}}} 
%\newcommand{\duesoon}[1]{{\sethlcolor{green}\hl{#1}}}
%\usepackage{mathrsfs}

% \newtheorem{theorem}{Theorem}
% \newtheorem{acknowledgement}[theorem]{Acknowledgement}
% \newtheorem{algorithm}[theorem]{Algorithm}
% \newtheorem{axiom}[theorem]{Axiom}
% \newtheorem{case}[theorem]{Case}
% \newtheorem{claim}[theorem]{Claim}
% \newtheorem{conclusion}[theorem]{Conclusion}
% \newtheorem{condition}[theorem]{Condition}
% \newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{criterion}[theorem]{Criterion}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{exercise}[theorem]{Exercise}
% \newtheorem{lemma}[theorem]{Lemma}
% %\newtheorem{notation}[theorem]{Notation}
% \newtheorem{problem}[theorem]{Problem}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{solution}[theorem]{Solution}
% \newtheorem{summary}[theorem]{Summary}
% %\newenvironment{proof}[1][Proof]{\textbf{#1.} }{\ \rule{0.5em}{0.5em}}

% \newtheorem{guess}{Definition}
%\newcommand{\Norder} {N}
\newcommand{\order}{\mathcal{O}}
% \newcommand{\Npoints} {N_p}
% \newcommand{\Nfaces} {N_{f}}
% \newcommand{\Nelements} {N_e}

%\newcommand{\eps}{\varepsilon}
%\newcommand{\Dweak}{\wt{D}}
\newcommand{\diff}[2] {\frac{\partial #1}{\partial #2}}
\newcommand{\dxx}[2] {\frac{\partial^2 #1}{\partial {#2}^2}}
\newcommand{\difft}[2] {\frac{d #1}{d #2}}
\newcommand{\dxxt}[2] {\frac{d^2 #1}{d {#2}^2}}
\newcommand{\lagrange}[1] {\frac{d #1}{dt}}
\newcommand{\lebesgue}{\parallel I \parallel}
\newcommand{\polysp}{\mathcal{P}_N}
\newcommand{\laplacian}{\nabla^2}
\newcommand{\divergence}{\nabla \cdot}
\newcommand{\inte}{\int_{\mbox{\footnotesize ${\Omega_e}$}}}
\newcommand{\intb}{\int_{\mbox{\footnotesize ${\Gamma_e}$}}}
\newcommand{\intce}{\int_{\mbox{\footnotesize ${\widehat{\Omega}_e}$}}}
\newcommand{\intcb}{\int_{\mbox{\footnotesize ${\widehat{\Gamma}_e}$}}}
\newcommand{\intg}{\int_{\mbox{\footnotesize ${\Omega}$}}}
\newcommand{\intgb}{\int_{\mbox{\footnotesize ${\Gamma}$}}}
\newcommand{\intv}{\int_{\mbox{\footnotesize ${\sigma}$}}}
% \newcommand{\sumv}{\sum_{K=1}^{N_{\mathrm{lev}}}}
% \newcommand{\sumk}{\sum_{L=1}^{K}}
% \newcommand{\sumN}{\sum_{i=1}^{N+1}}
% \newcommand{\half}{\frac{1}{2}}
% \newcommand{\inti}{\int_{\mbox{\footnotesize\sf I}}}
% \newcommand{\intbd}{\oint_{\mbox{\footnotesize ${\delta}$\sf D}}}
% \newcommand{\intbi}{\oint_{\mbox{\footnotesize ${\delta}$\sf I}}}
% \newcommand{\ldnorm}[1]{\left\| #1 \right\|_{\mbox{\footnotesize \sf D}} }
% \newcommand{\lonorm}[1]{\left\| #1 \right\|_{\Omega}}
% \newcommand{\spc}[1]{\mbox{\sf #1}}
% \newcommand{\ope}[1]{{\cal #1}}
% \newcommand{\mt}[1]{{\rm #1}}
% \newcommand{\dis}{\displaystyle}
% \newcommand{\ve}{\varepsilon}
% \newcommand{\ov}{\overline}
% \newcommand{\wt}{\widetilde}
% \newcommand{\wh}{\widehat}
% \newcommand{\Dhat}{\widehat{D}}
% \newcommand{\be}{\begin{equation}}
% \newcommand{\ee}{\end{equation}}
% \newcommand{\bea}{\begin{eqnarray*}}
% \newcommand{\eea}{\end{eqnarray*}}
% \newcommand{\Jace}{J^{(e)}}
% \newcommand{\Jacl}{J^{(l)}}
% \def\bepsilon{\mbox{\boldmath $\epsilon $}}
% \def\bpsi{\mbox{\boldmath $\psi $}}
% \def\bphi{\mbox{\boldmath $\phi $}}
% \def\bmu{\mbox{\boldmath $\mu $}}
% \def\Et{ \tilde{E} }
% \def\Ht{ \tilde{H} }
% \def\sdot{ \dot{\sigma} }

% \newcommand{\fstar}{f^{(*)}}

% \DeclareMathOperator{\Span}{span}
% \DeclareMathOperator{\Dim}{dim}

% \newcommand{\polyquad}{\mathcal{Q}_{N}}
% \newcommand{\polyP}{\mathcal{P}_{N}}
% \newcommand{\polyPnpm}{\mathcal{P}_{(N+M)}}
% \newcommand{\polyPd}{\mathcal{P}_{d}}
% \newcommand{\polyPnm}{\mathcal{P}_{N,M}}
% \newcommand{\polyPn}{\mathcal{P}_{N,0}}

\newcommand{\transpose}{^{\mathcal{T}}}

% \newcommand{\vecQ}{\vec{Q}}
% \newcommand{\vecQe}{\vec{Q}^{(e)}}
% \newcommand{\vecFe}{\vec{{F}}^{(e)}}
% \newcommand{\statevec}{\vec{Y}}
% \newcommand{\statevecN}{\vec{Y}_N^{(e)}}
% \newcommand{\statestage}{\vec{\mathcal{Y}}}
% \newcommand{\Ftensor}{\vec{F}(\qvector)}
% \newcommand{\FtensorN}{\vec{F}\left( \qvectorN \right)}
% \newcommand{\FtensorStar}{\vec{F}\left( \qvector_N^{(e,k)} \right)}
% \newcommand{\Svector}{S(\qvector)}
% \newcommand{\SvectorN}{S \left( \qvectorN \right)}
% \newcommand{\qref}{\vec{q}_0}
% \newcommand{\qvectorb}{\vec{q}_b}
% \newcommand{\qtt}{\vec{q}_{tt}}
% \newcommand{\qhat}{\widehat{\vec{q}}}
% \newcommand{\qhatb}{\widehat{\vec{q}}_b}
% \newcommand{\qelem}{q^{(e)}}
% \newcommand{\rhoref}{\rho_0}
% \newcommand{\piref}{\pi_0}
% \newcommand{\Thetaref}{\Theta_0}
% \newcommand{\Gref}{G_0}
% \newcommand{\Tref}{T_0}
% \newcommand{\thetaref}{\theta_0}
% \newcommand{\Pref}{{P}_0}
% \newcommand{\Eref}{{E}_0}
% \newcommand{\Href}{{h}_0}
% \newcommand{\rhohat}{\widehat{\rho}}
% \newcommand{\pihat}{\widehat{\pi}}
% \newcommand{\Phat}{\widehat{P}}
% \newcommand{\uvechat}{\widehat{{\mbox{\boldmath$u$\unboldmath}}}}
% \newcommand{\uhathat}{\widehat{\widehat{{\mbox{\boldmath$u$\unboldmath}}}}}
% \newcommand{\Uhat}{\widehat{{\mbox{\boldmath$U$\unboldmath}}}}
% \newcommand{\Uhathat}{\widehat{\widehat{{\mbox{\boldmath$U$\unboldmath}}}}}
% \newcommand{\thetahat}{\widehat{\theta}}
% \newcommand{\Thetahat}{\widehat{\Theta}}
% \newcommand{\Ehat}{\widehat{E}}
% \newcommand{\uhat}{\widehat{u}}
% \newcommand{\vhat}{\widehat{v}}
% \newcommand{\what}{\widehat{w}}
% \newcommand{\pitt}{\pi_{tt}}
% \newcommand{\rhott}{\rho_{tt}}
% \newcommand{\Ett}{E_{tt}}
% \newcommand{\Utt}{\vec{U}_{tt}}
% \newcommand{\uvectt}{\vec{u}_{tt}}
% \newcommand{\utt}{u_{tt}}
% \newcommand{\vtt}{v_{tt}}
% \newcommand{\wtt}{w_{tt}}
% \newcommand{\Ptt}{P_{tt}}
% \newcommand{\vecPtt}{\vec{P}_{tt}}
% \newcommand{\Thetatt}{\Theta_{tt}}
% \newcommand{\thetatt}{\theta_{tt}}
% %Projector Matrices
% \newcommand{\projmatrix}{\vec{\mathcal{P}}}
% \newcommand{\qmatrix}{\vec{\mathcal{Q}}}
% \newcommand{\pcmatrix}{\vec{\mathcal{P}}_C}
% \newcommand{\Cmatrix}{\left(\vec{\mathcal{C}}^{(e,f)}\right)\transpose}
% \newcommand{\Dmatrix}{\vec{D}^{(e)}}
% \newcommand{\Dwmatrix}{\wt{\vec{D}}^{(e)}}
% \newcommand{\Mmatrix}{M^{(e)}}
% \newcommand{\Fmatrix}{\vec{F}^{(e,l)}}
% \newcommand{\Gmatrix}{\mathcal{G}}
% \newcommand{\Umatrix}{\mathcal{U}^{(e,f)}}
% \newcommand{\amatrix}{\vec{\mathcal{A}}}
% \newcommand{\rmatrix}{\vec{\mathcal{R}}}
% %Vectors
% \newcommand{\nvector}{\wh{\vec{n}}_{\Gamma}}
% \newcommand{\nhat}{\wh{\vec{n}}}
% \newcommand{\ivector}{\wh{\vec{i}}}
% \newcommand{\jvector}{\wh{\vec{j}}}
% \newcommand{\kvector}{\wh{\vec{k}}}
% \newcommand{\rvector}{\wh{\vec{r}}}
% \newcommand{\svector}{\wh{\vec{s}}}
% \newcommand{\tvector}{\wh{\vec{t}}}
% \newcommand{\vvector}{\wh{\vec{v}}}
% \newcommand{\Qvector}{\vec{Q}}
% %Vectors
% \newcommand{\ur}{{u}^{(r)}}
% \newcommand{\us}{{u}^{(s)}}
% \newcommand{\ut}{{u}^{(t)}}
% \newcommand{\urtt}{{u}_{tt}^{(r)}}
% \newcommand{\ustt}{{u}_{tt}^{(s)}}
% \newcommand{\uttt}{{u}_{tt}^{(t)}}
% \newcommand{\urhat}{\widehat{u}^{(r)}}
% \newcommand{\ushat}{\widehat{u}^{(s)}}
% \newcommand{\uthat}{\widehat{u}^{(t)}}
%Other Operators
\newcommand{\grad}{\vec{\nabla}}
\newcommand{\Grad}{\vec{\nabla}}
%\newcommand{\Dskew}{\mathcal{D}}

% \def\bepsilon{\mbox{\boldmath $\epsilon $}}
% \def\bpsi{\mbox{\boldmath $\psi $}}
% \def\bphi{\mbox{\boldmath $\phi $}}
% \def\bmu{\mbox{\boldmath $\mu $}}
% \def\Et{ \tilde{E} }
% \def\Ht{ \tilde{H} }
% \def\sdot{ \dot{\sigma} }
%\renewcommand{\thetable}{\Roman{table}}
%\renewcommand{\thefigure}{\arabic{figure}}

%\DeclareMathOperator{\Span}{span}
%\DeclareMathOperator{\Dim}{dim}

% %Editing Commands
% \newcommand{\here}{ \textcolor{red}{YOU ARE HERE}}
% \newcommand{\red}[1]{ \textcolor{red}{#1}} 
% \newcommand{\blue}[1]{ \textcolor{blue}{#1}}
% \newcommand{\magenta}[1]{ \textcolor{magenta}{#1}}

% %Time-Integration
% \newcommand{\dt}{{\Delta t}}
% \newcommand\ST{\rule[-0.75em]{0pt}{2em}}
% \newcommand{\Sfunction}{\mathcal{S}}
% \newcommand{\Lfunction}{\mathcal{L}}
% \newcommand{\Nfunction}{\mathcal{N}}

% %DG Operators
% \newcommand{\average}[1]{ \left\{ #1 \right\} }
% \newcommand{\jump}[1]{ \llbracket #1 \rrbracket }

% %HDG Matrices
% \newcommand{\CCmatrix}{\mathcal{C}^{(e,k)}}
% \newcommand{\Jmatrix}{\mathcal{J}^{(e,k)}}
% \newcommand{\DDmatrix}{\wt{D}^{(e)}}
% \newcommand{\SSvector}{\mathcal{S}(q)}
% \newcommand{\cghdg}{cg\underline{\hspace{0.15cm}}to\underline{\hspace{0.15cm}}hdg}
% %\newcommand{\ul}{\underline{\hspace{0.15cm}}}
% \newcommand{\RRmatrix}{\mathcal{R}}

%Clima specific variables
% \newcommand{\etotal}{e^{\mathrm{tot}}}
% \newcommand{\Etotal}{E^{\mathrm{tot}}}
\newcommand{\Fvector}{\vec{{F}}}
% \newcommand{\Hvector}{\vec{\mathcal{H}}}
% \newcommand{\Pvector}{\vec{\mathcal{P}}}
% \newcommand{\Fadv}{\vec{{F}}^{\mathrm{adv}}}
% \newcommand{\Frad}{\vec{{F}}^{\mathrm{rad}}}
% \newcommand{\Fprecip}{\vec{{F}}^{\mathrm{precip}}}
% \newcommand{\Fdiff}{\vec{{F}}^{\mathrm{diff}}}
% \newcommand{\Fnondiff}{\vec{{F}}^{\mathrm{nondiff}}}
% \newcommand{\Tvector}{\vec{\mathcal{T}}}
\renewcommand{\Source}{\vec{\mathcal{S}}}

% %DG specific variables
% \newcommand{\gradvariables}{\vec{\mathcal{G}}}
% \newcommand{\diffusive}{\vec{\mathcal{D}}}

% %Units:
% \newcommand{\meters}{\,{\rm m}}

% \newcommand{\fxg}[1]{\textcolor{cyan}{(FXG: #1)}}
% \newcommand{\sm}[1]{\textcolor{green}{SM: #1}}

% \newcommand{\equa}[1]{(\ref{eq:#1})}
% \newcommand{\laeq}[1]{\label{eq:#1}}
% \newcommand{\figu}[1]{\ref{fig:#1}}
% \newcommand{\lafi}[1]{\label{fig:#1}}
% \newcommand{\si}[1]{\rm\scriptscriptstyle{#1}}
% \newcommand{\mbo}{\mbox{}}
% \newcommand{\Frac}[2]{\displaystyle{\frac{\displaystyle{#1}}{\displaystyle{#2}}}}
% \newcommand{\pal}[2]{\Frac{\partial #1}{\partial #2}}
% \newcommand{\pat}[1]{\pal{#1}{t}}
% \newcommand{\paxi}[1]{\pal{#1}{x_i}}
% \newcommand{\paxj}[1]{\pal{#1}{x_j}}
% \newcommand{\pxi}{\pal{\mbo}{x_i}}
% \newcommand{\pxj}{\pal{\mbo}{x_j}}
% \newcommand{\fmo}{\widetilde{U}}
% \newcommand{\fve}{\widetilde{u}}
% \newcommand{\Dt}{\Delta t}
% \newcommand{\Real}{\mathbb{R}}
% \newcommand{\climate}{{\tt ClimateMachine}}
% \newcommand{\clima}{{\tt Clima}}

% notation by International Standardization Organization:
% \DeclareMathAlphabet{\mathbfsf}{\encodingdefault}{\sfdefault}{bx}{sl}
% \newcommand{\vect}[1]{\boldsymbol{#1}}% vectors
% \newcommand{\uvect}[1]{\hat{\text{\textbf{#1}}}}% unit vectors
% \newcommand{\tensor}[1]{\mathbfsf{#1}}% tensors
% \newcommand{\D}{\text{d}}%total differential
% % plain notation:
% \renewcommand{\vect}[1]{#1}% vectors
% \renewcommand{\uvect}[1]{\hat{#1}}% unit vectors
% \renewcommand{\tensor}[1]{#1}% tensors
% \renewcommand{\D}{d}%total differential

% \newcommand{\Tcal}{\mathcal{T}}
% \newcommand{\Lcal}{\mathcal{L}}
% \newcommand{\Umbold}{\langle {\bf U} \rangle}
% \newcommand{\uijm}{\langle u_i u_j \rangle}

% \newcommand{\uum}{\langle u u \rangle}
% \newcommand{\uvm}{\langle u v \rangle}
% \newcommand{\uwm}{\langle u w \rangle}
% \newcommand{\vum}{\langle v u \rangle}
% \newcommand{\vvm}{\langle v v \rangle}
% \newcommand{\vwm}{\langle v w \rangle}
% \newcommand{\wum}{\langle w u \rangle}
% \newcommand{\wvm}{\langle w v \rangle}
% \newcommand{\wwm}{\langle w w \rangle}

% \newcommand{\Um}{\langle U \rangle}
% \newcommand{\Vm}{\langle V \rangle}
% \newcommand{\Wm}{\langle W \rangle}
% \newcommand{\Uim}{\langle U_i \rangle}
% \newcommand{\Ujm}{\langle U_j \rangle}
% \newcommand{\Rm}{\langle \rho \rangle}
% \newcommand{\Pm}{\langle p \rangle}
